CP-decomposition with Tensor Power Method for Convolutional Neural Networks Compression

Convolutional Neural Networks (CNNs) has shown a great success in many areas including complex image classification tasks. However, they need a lot of memory and computational cost, which hinders them from running in relatively low-end smart devices such as smart phones. We propose a CNN compression method based on CP-decomposition and Tensor Power Method. We also propose an iterative fine tuning, with which we fine-tune the whole network after decomposing each layer, but before decomposing the next layer. Significant reduction in memory and computation cost is achieved compared to state-of-the-art previous work with no more accuracy loss.

==> eqCompression2.tex <==
\begin{equation} \label{eq:Compression2}
E = \frac{TSD^2}{2RS + 2RD^2 + TR}
\end{equation}

==> eqCompression3.tex <==
\begin{equation} \label{eq:Compression3}
E = \frac{MN}{MR + RN}
\end{equation}

==> eqSpeedUp2.tex <==
\begin{equation} \label{eq:SpeedUp2}
C = \frac{TSD^2H'W'}{2RSHW + 2RD^2H'W' + TRH'W'}
\end{equation}

==> fig3wayCPDecomposition1.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{3wayCPDecomposition1.pdf}
	\caption{CP decomposition for a 3-way tensor.}
	\label{fig:3wayCPDecomposition1}
\end{figure}

==> fig4wayCPConvGroup2.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{4wayCPConvGroup2.pdf}
	\caption{Convolution with group = 2 in 4-ways CP decomposition}
	\label{fig:4wayCPConvGroup2}
\end{figure}

==> figAlexnet.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{Alexnet.pdf}
	\caption{AlexNet architecture \cite{krizhevsky2012imagenet}.}
	\label{fig:Alexnet}
\end{figure}

==> figConvCPDecomposition.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{ConvCPDecomposition.pdf}
	\caption{(a) Decomposing with 4-way rank-1 tensors, (b) with the spatial dimension untouched.}
	\label{fig:ConvCPDecomposition}
\end{figure}

==> figConvGroup2.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{ConvGroup2.pdf}
	\caption{Convolution with group = 2 in \textbf{(a)} original convolution and \textbf{(b)} CP decomposed convolution.}
	\label{fig:ConvGroup2}
\end{figure}

==> figGeneralStep.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8 \linewidth]{GeneralStep.pdf}
	\caption{Layer-by-layer decomposition and fine-tuning}
	\label{fig:GeneralStep}
\end{figure}

==> figImplementationSummary.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{ImplementationSummary.pdf}
	\caption{Implementation process.}
	\label{fig:ImplementationSummary}
\end{figure}

==> figSVD.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{SVD.pdf}
	\caption{Fully connected layer, with $M$ nodes of input and $N$ nodes of output, decomposition with SVD. (a) An $M \times N$ weights matrix is decomposed by SVD with rank $R$. The diagonal layer is first multiplied with left singular matrix. The final decomposition result consists of 2 matrices with size $M \times R$ and $R \times N$ consecutively. (b) A fully connected layer is decomposed to two fully connected layers with $M$, $R$, and $N$ nodes. } 
	\label{fig:SVD}
\end{figure}

==> figTPM.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{TPM.pdf}
	\caption{Tensor Power Method steps: \textbf{(a)} Find the first component to approximate the target tensor using coordinate descent. Then, find the residual tensor to be approximated in the next step. \textbf{(b)} Approximate the residual tensor to find the second component. Stop in this step for R=2 or find the residual tensor for the next step if R$>$2 until the number of components is equal to R.}
	\label{fig:TPM}
\end{figure}

==> table3waysvs4ways.tex <==
% Table generated by Excel2LaTeX from sheet 'SpatialComparison'
\begin{table*}[htbp]
	\centering
	\caption{Comparison between decomposing spatial dimension (4-way) and not decomposing spatial dimension (3-way). Weight and cost are number of weights and computational cost of Conv2.}
	\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|Y||Y|Y|Y|Y||Y|Y|Y|Y|}
		\hline
		\multirow{2}[4]{*}{} & \multicolumn{4}{c||}{R=100}    & \multicolumn{4}{c|}{R=200} \\
		\cline{2-9}          & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Weight} & \multicolumn{1}{c||}{Cost} & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Weight} & \multicolumn{1}{c|}{Cost} \\
		\hline
		\hline
		\multicolumn{1}{|l||}{Original} & 56.83 & 79.95 & 307K  & 223.9M & 56.83 & 79.95  & 307K  & 223.9M \\
		\hline
		\multicolumn{1}{|l||}{4-way} & 55.91 & 79.29 & 18K   & 24.9M & 56.03 & 79.20  & 37K   & 49.9M \\
		\multicolumn{1}{|l||}{(spatial dimension}& (-0.92) & (-0.66) & (6.05\%) & (11.14\%) & (-0.80) & (-0.75) & (12.11\%) & (22.29\%) \\
		\multicolumn{1}{|l||}{decomposed)}&&&&&&&&\\
		\hline
		\multicolumn{1}{|l||}{3-way} & 56.16 & 79.51 & 20K   & 25.7M & 56.49 & 79.71  & 40K   & 51.3M \\
		\multicolumn{1}{|l||}{(spatial dimension}& (-0.67) & (-0.44) & (6.54\%) & (11.46\%) & (-0.34) & (-0.24) & (13.09\%) & (22.93\%) \\
		\multicolumn{1}{|l||}{not decomposed)}&&&&&&&&\\
		\hline
	\end{tabularx}%
	\label{table:3waysvs4ways}%
\end{table*}%

\iffalse
\begin{table*}[t]
	\centering
	\begin{tabular}{ |p{2cm}||p{1.3cm}|p{1.3cm}|p{1.3cm}|p{1.3cm}||p{1.3cm}|p{1.3cm}|p{1.3cm}|p{1.3cm}| }
		\hline
		\multirow{2}{*}{} &\multicolumn{4}{c||}{R=50}&\multicolumn{4}{c|}{R=100} \\
		\cline{2-9}
		&\multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Weight} & \multicolumn{1}{c||}{Cost} &\multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Weight} & \multicolumn{1}{c|}{Cost} \\
		\hline\hline
		\multicolumn{1}{|l||}{Original}	& \multicolumn{1}{r|}{56.83}	& \multicolumn{1}{r|}{79.95}	& \multicolumn{1}{r|}{307K}	& \multicolumn{1}{r||}{223.9M}	& \multicolumn{1}{r|}{56.83}	& \multicolumn{1}{r|}{79.95}	& \multicolumn{1}{r|}{307K}	& \multicolumn{1}{r|}{223.9M}\\
		\hline
		\multicolumn{1}{|l||}{4-ways} & \multicolumn{1}{r|}{55.91} & \multicolumn{1}{r|}{79.29} 	& \multicolumn{1}{r|}{18K} 	& \multicolumn{1}{r||}{24.9M} & \multicolumn{1}{r|}{56.03}	& \multicolumn{1}{r|}{79.20} & \multicolumn{1}{r|}{37K} & \multicolumn{1}{r|}{49.9M}\\
		& \multicolumn{1}{r|}{(-0.92)} & \multicolumn{1}{r|}{(-0.66)} &&& \multicolumn{1}{r|}{(-0.80)} & \multicolumn{1}{r|}{(-0.75)} &&\\
		\hline
		\multicolumn{1}{|l||}{3-ways}	&  \multicolumn{1}{r|}{56.16} & \multicolumn{1}{r|}{79.51} 	& \multicolumn{1}{r|}{20K} & \multicolumn{1}{r||}{25.7M} & \multicolumn{1}{r|}{56.49}	& \multicolumn{1}{r|}{79.71} & \multicolumn{1}{r|}{40K} & \multicolumn{1}{r|}{51.3M}   \\
		& \multicolumn{1}{r|}{(-0.67)} & \multicolumn{1}{r|}{(-0.44)} &&& \multicolumn{1}{r|}{(-0.34)} & \multicolumn{1}{r|}{(-0.24)} &&\\
		\hline
	\end{tabular} 
	\caption{Comparison between decomposing spatial dimension (4-ways) and not decomposing spatial dimension (3-ways). Weight and cost are number of weights and computational cost of Conv2.}
	\label{}
\end{table*}
\fi

==> tableAllLayer.tex <==
% Table generated by Excel2LaTeX from sheet 'AllLayerImplementation'
\begin{table}[htbp]
	\centering
	\caption{All layer implementation comparison.}
	\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|X||r|r|r|r|}
		\hline
		\multirow{2}[2]{*}{} & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Weights}} & \multicolumn{1}{c|}{Comp.} \\
		& \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Acc} &       & \multicolumn{1}{c|}{Cost} \\
		\hline
		\hline
		Original & 56.83  & 79.95  & 61.0M & 724M \\
		\hline
		Tucker\cite{kim2015compression} & \multicolumn{1}{c|}{no} & 78.33  & 11.2M & 272M \\
		& \multicolumn{1}{c|}{data} & (-1.62) & (×5.46) & (×2.67) \\
		\hline
		This work & 54.81  & 78.48  & 8.7M  & 245M \\
		setting 01 & (-2.02) & (-1.47) & (×7.02) & (×2.95) \\
		\hline
		This work & 55.53  & 79.12  & 8.7M  & 245M \\
		setting 02 & (-1.30) & (-0.83) & (×7.02) & (×2.95) \\
		\hline
		This work & 54.06  & 77.70  & 8.5M  & 166M \\
		setting 03 & (-2.77) & (-2.25) & (×7.14) & (×4.36) \\
		\hline
		This work &       &       & 8.5M  & 166M \\
		setting 04 &       &       & (×7.14) & (×4.36) \\
		\hline
		
	\end{tabularx}%
	\label{table:AllLayer}%
\end{table}%

\iffalse
\begin{table}[t]
	\centering
	\begin{tabular}{ |l|r|r|r|r| }
		\hline
		\multirow{2}{*}{} 	& \multicolumn{1}{c|}{Top-1}	& \multicolumn{1}{c|}{Top-5}	& \multirow{2}{*}{Weights} 	& \multicolumn{1}{c|}{Computation} \\
		& \multicolumn{1}{c|}{Acc}	& \multicolumn{1}{c|}{Acc}	& & \multicolumn{1}{c|}{Cost}	   \\
		\hline\hline
		
		This work							& 54.94	& \textbf{78.44}	& \textbf{8.7M}	& \textbf{245M} \\
		&	(-1.89)	& \textbf{(-1.51)}	& \textbf{($\times$7.02)}	& \textbf{($\times$2.95)}	\\
		\hline
		
		Tucker\cite{kim2015compression}		& (no data)& 78.33	& 11M	& 272M	\\
		& & (-1.70)	& ($\times$5.46)	& ($\times$2.67)	\\
		\hline

	\end{tabular} 
	\caption{All layer implementation comparison}
	\label{}
\end{table}
\fi

==> tableAllLayer2.tex <==
% Table generated by Excel2LaTeX from sheet 'AllLayerImplementation'
\begin{table}[htbp]
	\centering
	\caption{All layer implementation comparison.}
	\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|X||r|r|r|r|}
		\hline
		\multirow{2}[2]{*}{} & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Weights}} & \multicolumn{1}{c|}{Comp.} \\
		& \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Acc} &       & \multicolumn{1}{c|}{Cost} \\
		\hline
		\hline
		Original & 56.83  & 79.95  & 61.0M & 724M \\
		\hline
		Tucker \cite{kim2015compression} & \multicolumn{1}{c|}{no} & 78.33  & 11.2M & 272M \\
		& \multicolumn{1}{c|}{data} & (-1.62) & ($\times$5.46) & ($\times$2.67) \\
		\hline
		This work & 55.53  & 79.12  & 8.7M  & 245M \\
		& (-1.30) & (-0.83) & ($\times$7.02) & ($\times$2.95) \\
		\hline
	\end{tabularx}%
	\label{table:AllLayer2}%
\end{table}%

==> tableNLSvsTPM.tex <==

% Table generated by Excel2LaTeX from sheet 'Sheet9'
\begin{table*}[htbp]
	\centering
	\caption{Comparison of NLS and TPM top-5 accuracy loss results without fine tuning (No FT) and with fine tuning (FT). Fine tuning is done in 15 epochs with base learning rate 0.001 and decrease it by factor of 10 every 5 epochs. NLS value result was approximated from Figure 2 graph in \cite{lebedev2014speeding}. In R=100 without fine tuning, it is not clear whether NLS or TPM is better since NLS value was approximated. In R=100 with fine tuning, TPM is better which gives more compression level with loss less than 1\%. For R=200 without fine tuning experiment, it is clear enough that NLS is better. In fine tuned R=200 result, NLS has range 0.4 until 0.5 so it still slightly better than the TPM. But both of the results still achieved less than 1\% loss.}
	\begin{tabularx}{\linewidth}{|X||Y|Y||Y|Y||Y|Y||Y|Y||Y|Y|}
		\hline
		\multicolumn{1}{|c||}{\multirow{2}[4]{*}{Algorithm}} & \multicolumn{2}{c||}{R=50} & \multicolumn{2}{c||}{R=100} & \multicolumn{2}{c||}{R=140} & \multicolumn{2}{c||}{R=200} & \multicolumn{2}{c|}{R=300}\\
		\cline{2-11} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c||}{FT} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c||}{FT} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c||}{FT} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c||}{FT} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c|}{FT}\\
		\hline
		\hline
		CP-NLS\cite{lebedev2014speeding} & - & - & \url{~}79   & \url{~}19   & 3.21 & \url{~}1.3 & 0.97 & \url{~}0.45 & 0.30 & -\\
		\hline
		CP-TPM  & 79.23 & 0.99 & 79.38 & 0.66 & 79.37 & 0.59 & 79.44 & 0.75 & 79.43 & 0.65 \\
		\hline
	\end{tabularx}%
	\label{table:NLSvsTPM}%
\end{table*}%

\iffalse
\begin{table}[h]
	\centering
	\begin{tabular}{ |p{1.3cm}||p{1.1cm}|p{1.1cm}||p{1.1cm}|p{1.1cm}| }
		\hline
		\multirow{2}{*}{Algorithm} &\multicolumn{2}{|c||}{R=100}&\multicolumn{2}{c|}{R=200} \\
		\cline{2-5}
		&\multicolumn{1}{|c|}{No FT} & \multicolumn{1}{c||}{FT} & \multicolumn{1}{c|}{No FT} & \multicolumn{1}{c|}{FT} \\
		\hline\hline
		NLS\cite{lebedev2014speeding}	&  \multicolumn{1}{|r|}{79}	& \multicolumn{1}{r||}{19} 	& \multicolumn{1}{r|}{\textbf{1}} 	& \multicolumn{1}{|r|}{\textbf{0.45}}	\\
		\hline
		TPM	& \multicolumn{1}{|r|}{79.44}	& \multicolumn{1}{r||}{\textcolor{red}{\textbf{0.75}}}	& \multicolumn{1}{r|}{79.45} & \multicolumn{1}{|r|}{0.65}		\\
		\hline
	\end{tabular} 
	\caption{Comparison of NLS and TPM top-5 accuracy loss results without fine tuning (No FT) and with fine tuning (FT). NLS value result was approximated from Figure 2 graph in \cite{lebedev2014speeding}. In R=100 without fine tuning, it is not clear whether NLS or TPM is better since NLS value was approximated. In R=100 with fine tuning, TPM is better which gives more compression level with loss less than 1\%. For R=200 without fine tuning experiment, it is clear enough that NLS is better. In fine tuned R=200 result, NLS has range 0.4 until 0.5 so it still slightly better than the TPM. But both of the results still achieved less than 1\% loss.}
	\label{}
\end{table}
\fi

==> tableRank.tex <==
\begin{table}[htbp]
	\centering
	\caption{Rank calculated from the top-5 accuracy loss.}
	
	
	\begin{tabular}{|r||l|r|r|r|}
		
			\hline
			& \multicolumn{1}{c|}{\multirow{2}[0]{*}{Layer}} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{\multirow{2}[0]{*}{Rank}} \\
			&       & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Loss} &  \\
		
	    	\hline\hline
	    	
	    	& Conv1 & 74.45  & 5.50  & 71 \\
	    	\cline{2-5}          & Conv2 & 68.00  & 11.95  & 152 \\
	    	\cline{2-5}    \multicolumn{1}{|c||}{Conv} & Conv3 & 67.66  & 12.29  & 157 \\
	    	\cline{2-5}    \multicolumn{1}{|c||}{(Ave=150)} & Conv4 & 66.18  & 13.77  & 176 \\
	    	\cline{2-5}          & Conv5 & 64.68  & 15.27  & 194 \\
	    	\cline{2-5}          & \textbf{Total} &       & \textbf{58.78} & \textbf{750} \\
	    	\hline
	    	\hline
	    	& FC6   & 51.47 & 28.48  & 364 \\
	    	\cline{2-5}    \multicolumn{1}{|c||}{FC} & FC7   & 58.39 & 21.56  & 275 \\
	    	\cline{2-5}    \multicolumn{1}{|c||}{(Ave=300)} & FC8   & 59.51 & 20.44  & 261 \\
	    	\cline{2-5}          & \textbf{Total} &       & \textbf{70.48} & \textbf{900} \\
	    	\hline
	 \end{tabular}%
	    
	
	\label{table:Rank}%
\end{table}%


==> tableRankConv.tex <==
% Table generated by Excel2LaTeX from sheet 'RankProportion'
\begin{table*}[htbp]
	\centering
	\caption{Finding rank for convolution layer. Desired rank value is arbitrary. Rounded rank will be used for the experiment.}
	\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|X|Y|Y||Y|Y|Y||Y|Y|Y|}
		\hline
		\multicolumn{1}{|c|}{\multirow{2}[1]{*}{Layer}} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c||}{Top-5} & \multicolumn{1}{c|}{Desired} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{Rank }} & \multicolumn{1}{c||}{Rounded} & \multicolumn{1}{c|}{Desired} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{Rank }} & \multicolumn{1}{c|}{Rounded} \\
		& \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c||}{ Loss} & \multicolumn{1}{c|}{Rank} &       & \multicolumn{1}{c||}{Rank} & \multicolumn{1}{c|}{Rank} &       & \multicolumn{1}{c|}{Rank} \\
		
		\hline\hline
		
		Conv1 & 70.55  & 9.40  & 150   & 99.20  & \textbf{99} & 100   & 66.13  & \textbf{66} \\
		\hline
		Conv2 & 68.00  & 11.95  & 150   & 126.16  & \textbf{126} & 100   & 84.11  & \textbf{84} \\
		\hline
		Conv3 & 59.28  & 20.67  & 150   & 218.14  & \textbf{218} & 100   & 145.42  & \textbf{145} \\
		\hline
		Conv4 & 66.18  & 13.77  & 150   & 145.31  & \textbf{146} & 100   & 96.87  & \textbf{97} \\
		\hline
		Conv5 & 64.68  & 15.27  & 150   & 161.20  & \textbf{161} & 100   & 107.47  & \textbf{108} \\
		\hline
		\hline
		Total &       & 71.06  & 750   & 750   & 750   & 500   & 500   & 500  \\
		\hline
	\end{tabularx}%
	\label{table:RankConv}%
\end{table*}%


\iffalse
\begin{table}[t]
	\centering
	\begin{tabular}{ |l|r|r|r|r|r| }
		\hline
		\multirow{2}{*}{Layer} 	& \multicolumn{1}{c|}{Top-5}	& \multicolumn{1}{c|}{Top-5}	& \multicolumn{1}{c|}{Desired}	& \multirow{2}{*}{Rank} 	& \multicolumn{1}{c|}{Rounded} \\
		& \multicolumn{1}{c|}{Acc}	& \multicolumn{1}{c|}{Loss}	& \multicolumn{1}{c|}{Rank}	&  	& \multicolumn{1}{c|}{Rank} \\
		\hline\hline
		
		Conv1	& 70.55	& 9.40	& 150	& 99.21		& \textbf{99}  \\
		\hline
		Conv2	& 68.00	& 11.95	& 150	& 126.13	& \textbf{126} \\
		\hline
		Conv3	& 59.28	& 20.67	& 150	& 218.16	& \textbf{218} \\
		\hline
		Conv4	& 66.18	& 13.77	& 150	& 145.33	& \textbf{146} \\
		\hline
		Conv5	& 64.68	& 15.27	& 150	& 161.17	& \textbf{161} \\
		\hline
		Total	&		& 71.06	& 750	& 750		& 750 \\
		\hline
		
	\end{tabular} 
	\caption{Finding rank for convolution layer. Desired rank value is arbitrary. Rounded rank will be used for the experiment.}
	\label{}
\end{table}
\fi

==> tableRankFC.tex <==
% Table generated by Excel2LaTeX from sheet 'RankProportion'
\begin{table}[htbp]
	\centering
	\caption{Finding rank for fully connected layer. Desired rank value is arbitrary. Rounded rank will be used for the experiment.}
	\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|X|Y|Y||r|Y|r|}
		\hline
		\multicolumn{1}{|c|}{\multirow{2}[1]{*}{Layer}} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c||}{Top-5} & \multicolumn{1}{c|}{Desired} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{Rank }} & \multicolumn{1}{c|}{Rounded} \\
		& \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c||}{ Loss} & \multicolumn{1}{c|}{Rank} &       & \multicolumn{1}{c|}{Rank} \\
		
		\hline\hline
		
		FC6   & 32.69  & 47.26  & 300   & 338.16  & \textbf{338} \\
		\hline
		FC7   & 40.06  & 39.89  & 300   & 285.41  & \textbf{285} \\
		\hline
		FC8   & 41.32  & 38.63  & 300   & 276.44  & \textbf{277} \\
		\hline
		\hline
		Total &       & 125.78  & 900   & 900   & 900  \\
		\hline
	\end{tabularx}%
	\label{table:RankFC}%
\end{table}%



\iffalse
\begin{table}[t]
	\centering
	\begin{tabular}{ |l|r|r|r|r|r| }
		\hline
		\multirow{2}{*}{Layer} 	& \multicolumn{1}{c|}{Top-5}	& \multicolumn{1}{c|}{Top-5}	& \multicolumn{1}{c|}{Desired}	& \multirow{2}{*}{Rank} 	& \multicolumn{1}{c|}{Rounded} \\
		& \multicolumn{1}{c|}{Acc}	& \multicolumn{1}{c|}{Loss}	& \multicolumn{1}{c|}{Rank}	&  	& \multicolumn{1}{c|}{Rank} \\
		
		\hline\hline
		
		FC6		& 32.69	& 47.26	& 300	& 338.16	& \textbf{338} \\
		\hline
		FC7		& 40.06	& 39.89	& 300	& 285.41	& \textbf{285} \\
		\hline
		FC8		& 41.32	& 38.63	& 300	& 276.44	& \textbf{277} \\
		\hline
		Total	&		& 125.78& 900	& 900		& 900 \\
		\hline
		
	\end{tabular} 
	\caption{Finding rank for fully connected layer. Desired rank value is arbitrary. Rounded rank will be used for the experiment.}
	\label{}
\end{table}
\fi

==> tableRankProportionComparison.tex <==
% Table generated by Excel2LaTeX from sheet 'RankComparison'
\begin{table*}[htbp]
  \centering
  \caption{Rank proportion comparison with top-5 loss and top-1 loss with desired average rank 150. There is no significant different in the rank result (the Rounded Rank).}
    \begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}|X|r||Y|Y|Y|Y||Y|Y|Y|Y|}
    \hline
    \multicolumn{1}{|c|}{\multirow{3}[4]{*}{Layer}} & \multicolumn{1}{c||}{\multirow{3}[4]{*}{Desired Rank}} & \multicolumn{4}{c||}{Top-5}   & \multicolumn{4}{c|}{Top-1} \\
\cline{3-10}          &       & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{Top-5} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Rank }} & \multicolumn{1}{c||}{Rounded} & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{Top-1} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Rank }} & \multicolumn{1}{c|}{Rounded} \\
          &       & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{ Loss} &       & \multicolumn{1}{c||}{Rank} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{Loss} &       & \multicolumn{1}{c|}{Rank} \\
    \hline
    \hline
    Conv1 & 150   & 70.55  & 9.40  & 99.20  & \textbf{99} & 45.33 & 11.498 & 105.18  & \textbf{105} \\
    \hline
    Conv2 & 150   & 68.00  & 11.95  & 126.16  & \textbf{126} & 43.086 & 13.742 & 125.71  & \textbf{126} \\
    \hline
    Conv3 & 150   & 59.28  & 20.67  & 218.14  & \textbf{218} & 34.434 & 22.394 & 204.86  & \textbf{205} \\
    \hline
    Conv4 & 150   & 66.18  & 13.77  & 145.31  & \textbf{146} & 40.788 & 16.04 & 146.73  & \textbf{147} \\
    \hline
    Conv5 & 150   & 64.68  & 15.27  & 161.20  & \textbf{161} & 38.516 & 18.312 & 167.52  & \textbf{167} \\
    \hline\hline
    Total & 750   &       & 71.06  & 750   & 750   &       & 81.986 & 750   & 750 \\
    \hline
    \end{tabularx}%
  \label{table:RankProportionComparison}%
\end{table*}%


==> tableSetting.tex <==
% Table generated by Excel2LaTeX from sheet 'RankList'
\begin{table}[htbp]
  \centering
  \caption{Settings used in all layer implementation. Rank is desired or average rank. Epoch is number of training epoch for last layer and the other layers.}
    \begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}|l||Y|Y||Y|r|}
    \hline
    \multicolumn{1}{|c||}{\multirow{2}[4]{*}{Setting}} & \multicolumn{2}{c||}{Rank} & \multicolumn{2}{c|}{Epoch} \\
\cline{2-5}          & \multicolumn{1}{c|}{Conv} & \multicolumn{1}{c||}{FC} & \multicolumn{1}{c|}{Others} & \multicolumn{1}{c|}{Last Layer} \\
    \hline
    \hline
    01    & 150   & 300   & 3     & 15 \\
    \hline
    02    & 150   & 300   & 15    & 15 \\
    \hline
    03    & 100   & 300   & 3     & 15 \\
    \hline
    04    & 100   & 300   & 15    & 15 \\
    \hline
    \end{tabularx}%
  \label{table:Setting}%
\end{table}%

